Lightweight Inter-transaction Caching with Precise Clocks and Dynamic Self-invalidation

Distributed, transactional storage systems scale by sharding data across servers. However, workload-induced hotspots result in contention, leading to higher abort rates and performance degradation. We present KAIROS, a transactional key-value storage system that leverages client-side inter-transaction caching and sharded transaction validation to balance the dynamic load and alleviate workload-induced hotspots in the system. KAIROS utilizes precise synchronized clocks to implement self-invalidating leases for cache consistency and avoids the overhead and potential hotspots due to maintaining sharing lists or sending invalidations. Experiments show that inter-transaction caching alone provides 2.35x the throughput of a baseline system with only intra-transaction caching; adding sharded validation further improves the throughput by a factor of 3.1 over baseline. We also show that lease-based caching can operate at a 30% higher scale while providing 1.46x the throughput of the state-of-the-art explicit invalidation-based caching.

==> implementation.tex <==
\section{Implementation}\label{sec:implementation}
Figure~\ref{fig:design_space} shows the design choices for caching and validation. Each combination of choices represents a point in the design space for \sysname{}. By restricting validation to the server, we were able to implement different cache designs, and explore trade-offs more practically. 
 
\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{design_space.png}
\caption{Design choices for caching and validation.~\Srihari{replace placeholder with pdf.}}
\label{fig:design_space}
\end{figure}

\parab{Server-side Caching}: We still have DRAM accesses on the server, but no offloading of transactional validation. Also not sure if we get the nice spatial locality properties of the sharer cache in the case of transactional applications, or distributed operations that access keys across multiple shards. 

\parab{Client-side Non-Coherent Caching}: Cannot validate; good read performance; will probably do badly under even a moderately write-heavy workload (Ex.write ratio of 20\%) 

\parab{Client-side Single-Copy Caching}: No sharers, keys are assigned using consistent hashing. pros: no directory or invalidation costs; no expensive(?) lease calculations; 

\parab{Client-side Coherent Caching}: Each client library maintains a
local cache instance and reads data from it. To
support local validation, the client also sends a
GET request to shards (off the critical path) and
the shards return version information that aids
local validation. This approach provides latency
benefits but no distribution in validation load.

==> system_old.tex <==
\section{\sysname: A Transactional Key-Value Storage System}
\label{sec:architecture}
This section presents \sysname, a transactional key-value storage system that leverages client-side inter-transaction caching and validation to improve performance and balance the dynamic load across servers.

\subsection{System architecture}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{system.pdf}
\caption{\sysname architecture}
\label{fig:architecture}
\end{figure}

Figure~\ref{fig:architecture} shows the architecture of \sysname. The \sysname design targets an intra-data center client/server storage model. Data is stored on DRAM / NVM (e.g., SSDs) on the storage servers. The key space is sharded across the storage servers, and each shard is replicated for availability and fault tolerance. Applications run on one or more multi-tenant client servers. A frontend load balancer (e.g., Slicer~\cite{adya2016slicer}) distributes user transactions across application instances on different client servers, while balancing load or exploiting any locality of accesses.

\sysname uses optimistic concurrency control (OCC~\cite{kung1981on}) adapted to a client/server setting~\cite{adya1995efficient} to support ACID transactions. OCC is an alternative to locking (two-phase locking or 2PL): OCC enhances concurrency relative to 2PL, and is not prone to 2PL's blocking and deadlocks.  OCC systems {\it validate} each transaction $T$ before commit by comparing $T$'s timestamped data accesses---$T$'s {\it read set} and {\it write set}---to those of other transactions 
to identify any access conflicts that violate a consistent transaction ordering (e.g., serializable ordering). Conflicting transactions are aborted and then restarted at the client. Validation of transactions in OCC is typically performed on the storage servers~\cite{adya1995efficient, zhang2015building, misra2017enabling}; however, \sysname offloads the validation workload to client-side validators, and the storage servers are involved in a backup validation path when the validators do not have the requisite state to validate a transaction.

\sysname also allows inter-transaction caching on the client. Each client cache operates independently and popular data may be replicated across multiple client caches. Client-side caching can reduce network traffic and latency of transactions because reads that hit the local cache do not require any remote communication with the server. Caching can also help balance the dynamic load across servers~\cite{fan2011small,li2016switchkv}. However, maintaining consistency across client caches is a challenge when a cached key is updated. Prior work~\cite{adya1995efficient} has proposed an invalidation-based approach to cache consistency where servers track sharers (client caches with a copy of the key) and send out invalidation requests to sharers when the key is updated. The downside of this approach is the storage cost for tracking sharers, performance overhead of broadcasting invalidations and impact on scalability. Due to the complexity in maintaining cache consistency, distributed transactional storage systems rarely allow caching of data across multiple servers~\cite{yu2018sundial}.

\sysname uses leases for addressing the problem of maintaining client cache consistency. Storage servers hand out leases for caching frequently-read keys and do not track sharers nor broadcast any invalidations; a cached key is {\em self-invalidated} by client caches on lease expiration. Lease durations are probabilistic and are predicted based on the inter-access (read and write) times of keys. A key may be updated while a lease is still active and cause stale hits on caches, but system safety is not compromised because all transactions are validated before commit. However, stale hits hinder forward progress because a transaction that reads any stale data is aborted at the time of validation, which leads to wastage of resources and lower commit rates. The aggressiveness of a cache consistency mechanism has an impact on the number of stale hits and thereby on forward progress. We discuss client cache consistency mechanisms in Section~\ref{sec:caching}.

Each key in a client cache is associated with a value, version timestamp ($ts_{version}$), lease end time ($ts_{leaseEndTime}$) and freshness timestamp ($ts_{freshness}$). $ts_{version}$ is the timestamp of the transaction that wrote the version, $ts_{leaseEndTime}$ indicates the time at which the entry will be self-invalidated from the cache. $ts_{freshness}$ indicates the latest timestamp for which the client knows that the cached version is fresh i.e., there are no superseding writes with timestamp $t$ between $ts_{version}$ $<$ t $<$ $ts_{freshness}$.

\PM{Talk about watermarks}

\subsection{Transaction protocol}
Each application instance runs a \sysname library that exposes a transactional key/value storage API and issues transactions to the system. The library coordinates with a global master to map each key to a validator/storage shard using standard techniques (e.g., consistent hashing \cite{karger1997consistent}). The master maintains the shard maps based on its global view of participating servers. The master can be implemented using standard techniques (e.g., Apache Zookeeper~\cite{hunt2010zookeeper}).

Below is the application API to the \sysname client library. Timestamp $t_{current}$ represents the client's local view of the current time, as given by PTP.
\begin{itemize}
\setlength\itemsep{0pt}
\setlength\parsep{0pt}
\sloppy
\item {\bf beginTransaction()}:  Start a new transaction $T$ and initialize an empty read and write set for $T$.
\item {\bf abortTransaction()}: Discard the read and write set maintained for $T$ and remove all state.
\item {\bf commitTransaction() $\rightarrow$ Success / Fail}: Assign freshness and commit timestamp to $T$ and initiate the commit protocol, which can either succeed or fail.
\item {\bf put(key, value)}: Buffer the key-value pair, add key to the $T$'s write set.
\item {\bf get(key) $\rightarrow$ value}: Return a value for the key, add key to the $T$'s read set.
\end{itemize}

\begin{figure}[t]
    \begin{algorithm}[H]
    \begin{algorithmic}[1]
  	\scriptsize
    \Procedure {read}{T, key}
    	\If {key $\in$ T.writeSet}
        	\State return T.writeSet[key].value
        \ElsIf {key $\in$ T.readSet}
        	\State return T.readSet[key].value
        \Else
        	\If {key $\notin$ Cache \textbf{or} Cache[key].lts $>$ $t_{current}$}
            	\State Cache[key].\{value, vts, lts, fts\} = get\_from\_server(key)
            \EndIf
            \State T.readSet[key].\{value, vts, fts\} = Cache[key].\{value, vts, fts\}
            \State return T.readSet[key].value
        \EndIf
    \EndProcedure
    \Statex
	\Procedure {write}{T, key, value}
    \State T.writeSet[key].value = value
    \EndProcedure
	\caption{Processing phase of a transaction $T$. For brevity, $ts_{version}$ = vts, $ts_{leaseEndTime}$ = lts, $ts_{freshness}$ = fts}
    \label{alg:execute}
    \end{algorithmic}
    \end{algorithm}
\end{figure}

\sysname executes transactions in a similar manner to other client/server transaction systems with OCC~\cite{adya1995efficient, zhang2015building,ding2015centiman,lee2015implementing}. Algorithm~\ref{alg:execute} shows how a transaction $T$'s reads and write requests are handled during the processing phase; all operations are tracked in $T$'s read and write set, which are maintained in client memory during the entire execution of $T$. For a read request, a value is returned if the key exists in the $T$'s write or read set. Otherwise, the transaction checks the local cache for the key. On a cache miss, the read request is sent to the remote server and the returned data is placed in the local cache; for a read request, the server returns the value, $ts_{version}$, $ts_{leaseEndTime}$ and $ts_{freshness}$. $ts_{freshness}$ is set to max of the timestamp of the returned version and server's view of the global watermark, i.e., $ts_{freshness} = max(ts_{version}, ts^{global}_{watermark})$. After fetching the data from the server or on a cache hit, $T$'s read set is updated with the cached data before the value is returned to the application. For each key read in the transaction, the read set tracks the value, $ts_{version}$ and $ts_{freshness}$. All transaction writes during the processing phase are buffered and made visible only after a transaction commits. 

The processing phase finishes when the application invokes {\em commitTransaction}. Before initiating the commit process, the client assigns a freshness and commit timestamp to the transaction $T$. The freshness timestamp ($T_{freshness}$) is the minimum freshness timestamp from all keys in the read set i.e., $T_{freshness} = \displaystyle \min_{key \in readSet} key.fts$. The commit timestamp ($T_{commit}$) depends on the type of transaction (read-only or read-write); for a read-only transaction, the commit timestamp is max freshness timestamp from all keys in the read set i.e., $T_{commit} = \displaystyle \max_{key \in readSet} key.fts$ and for a read-write transaction, $T_{commit} = t_{current}$, where $t_{current}$ is the current time on the client. After assigning the timestamps, the client initiates and coordinates the two-phase commit (2PC) protocol; the 2PC participants include the storage servers and validators for all keys in either set. The client pushes modified values for keys in the write set to their servers on a commit request, and not before (\S\ref{sec:validation}).

\begin{figure}[tb]
\centering
 \includegraphics[height=2in,keepaspectratio]{./figures/2PC.pdf} 
 \caption{Two Phase Commit for a read-write transaction. Read-only transactions require only 1 phase (validate)}
\label{fig:2PC}
\end{figure}

\subsection{Validation}
\label{sec:validation}
\begin{figure}[t]
    \begin{algorithm}[H]
      \begin{algorithmic}[1]
       \scriptsize
       \Procedure {validate}{transaction} 
         \For {each (key, version) $\in$ txn.readSet}
          \If {key.prepared $\neq$ NONE}
              \State return ABORT
           \ElsIf {key.latestCommitted $\neq$ version}
           	  \State return ABORT
           \EndIf
         \EndFor
         \State newVersion = transaction.commitTimestamp
         \For {each (key, version) $\in$ transaction.writeSet} 
          \If {key.preparedWrite $\neq$ NONE}
              \State return ABORT 
           \ElsIf {key.preparedRead $\geq$ newVersion}
           	  \State return ABORT
           \ElsIf {key.latestCommitted $\geq$ newVersion}
              \State return ABORT
           \EndIf
           \If {newVersionTS $<$ key.leaseEndTime}
           \State invalidateSharers(key)
           \EndIf
         \EndFor
         \State return COMMIT
          \EndProcedure
        \caption{Validation Algorithm}
        \label{alg:validation}
        \end{algorithmic}
        \end{algorithm}
\end{figure}
\normalsize

When an application issues a commit, the transaction library client begins a 2PC protocol and acts as the coordinator. The client performs the following operations to validate the requested commit:

\myparagraph{Read-only transaction}
.  client sends a {\em validate} request to all participant validators; each validator receives keys in the read set for key shards that it controls, and a list of other participant validators. Each validator validates keys against the respective version stamps to decide if there are any conflicts that violate strict serializability, as shown in Algorithm~\ref{alg:validation}, and returns the decision (SUCCESS/ABORT) back to the client. Although not shown in the algorithm, the validator also updates the $ts_{preparedRead}$ field of all keys for all successfully validated transactions. The client accumulates the response from all validators and if there are any ABORTs, the client returns an ABORT back to the application. If all requests are successfully validated, it returns a SUCCESS back to the application.

\myparagraph{Read-write transaction}
Figure~\ref{fig:2PC} shows an example read-write transaction with a two phase commit (2PC) protocol. In phase 1, similar to a read-only transaction, the client sends a {\em validate} request to all participant validators; each validator receives keys in the read {\em and write sets} for key shards that it controls, and a list of other participant validators. Each validator validates the keys using Algorithm~\ref{alg:validation}. As seen in the algorithm (lines 18-20), for all keys successfully validated in the write set, a validator also invalidates any sharers if timestamp of new version is less than lease end time. Finally, each validator returns a response (SUCCESS/ABORT) back to the client.

Simultaneously with the validate request, the client also sends a {\em replicate} request to the primary of all participant storage shards; each primary receives keys in the {\em write set} for key shards that it controls. The primary propagates the replicate request to all backups  and waits for {\em f (out of 2f)} backups to respond before it returns a response to the client.

The client accumulates the responses for the validate requests from all participant validators. It also waits for the response for all replicate requests sent to primaries of participant storage shards. Finally, if there are any ABORTs, the client issues an ABORT to all primaries and validators, and returns the abort to the application. If all keys are successfully validated, then the client issues a COMMIT to each primary and validator, and returns SUCCESS to the application.

\subsection{Watermarks and version management}


\subsection{Recovery}
This section describes what happens if a client, validator or storage server (e.g., a primary) fails during the process of committing a transaction. \sysname assumes fail-stop (non-byzantine) failures.\\

\myparagraph{Client failure} If the client fails during 2PC, then the participants (validators and primaries) time out waiting for a commit or abort decision for a prepared transaction $T$. $T$ is blocked until its commit/abort status is known.  This situation does not affect any transactions operating on  key sets that are disjoint from $T$'s read/write sets. However, the validators are forced to abort any transaction that attempts to read/write any of the keys in  $T$'s read or write set, until $T$'s commit/abort status is known.  In such a case, one of the participating validators is designated as a backup coordinator for $T$. The backup coordinator can use the Cooperative Termination Protocol (CTP) ~\cite{bernstein1987concurrency} to determine if $T$ should commit.  The backup coordinator queries the other participating validators for the status of $T$, and takes appropriate action. The states are {\em Received Commit, Received Abort, Prepared, Sent Commit, Sent Abort} and the actions can be any of the following:

\begin{enumerate}
\setlength\itemsep{0pt}
\setlength\parsep{0pt}
\item If any validator received a commit or abort then $T$ should be committed or aborted since the client made a decision only after receiving a response from all the validators.
\item If any validator did not receive a prepare request for $T$, then all primaries can agree to abort $T$ because the client does not commit a transaction until it receives a response from all validators for its shards.
\item If any validator responded with ABORT to the prepare request, then all validators abort $T$.
\item If all validators responded SUCCESS for the prepare request then the backup coordinator commits $T$.
\end{enumerate}

\myparagraph{Storage shard failure}
If a backup replica of a participant shard fails during 2PC, it does not block any transaction as long as a majority of replicas for a shard are available to store transactions. However if a primary of a participant shard fails then it would block all transactions involving that shard. A new primary must be elected (failover) in order to unblock any running transactions and resume service.

The new primary can always reach a consistent state if there are $f+1$ replicas available (out of $2f+1$), which are needed for a majority quorum. For $f+1$ available replicas, there must always be at least one replica that has seen any given transaction committed or prepared by the previous primary. Therefore the new primary has access to all the transactions and can rebuild the data versions and transaction table by merging the updates from all the replicas. If a transaction prepare or commit record is not present on at least one replica at recovery, then the previous primary could not have obtained a majority for the operation, and therefore could not have acknowledged the request.  In this case, 2PC recovery restores the state of these transactions, as detailed above (CTP). 

The new primary can then apply all the successfully committed transactions without any validation. For all {\em replicated} transaction, the new primary must contact the participant validators to determine whether the transaction committed.  The transaction is committed or aborted if any validator responds with a COMMIT or ABORT, respectively.  If all participant validators respond with a prepared status then the transaction is still outstanding and should be committed and a response sent to the client.\\

\myparagraph{Validator failure}
If a participant validator fails during 2PC then the corresponding storage shards take the responsibility of validating transactions for keys owned by the validator. The primaries of storage shards can validate all outstanding read-only transactions but might not have enough state to validate read-write transactions. 

Specifically, the primary may not have the correct $ts_{preparedRead}$ for a key since there might be a read-only transaction that updated this field on the failed validator but the storage shard did not receive any request for this transaction. Validating any read-write transaction without these values can violate serializability. Consider the following scenario: a read-only transaction $T_a$ read key $K$ and was successfully committed with a timestamp $t_2$. Now the validator for key $K$ fails, and the primary allows a read-write transaction $T_b$ to commit that creates a new version of $K$ with timestamp $t_1$ ($t_0 < t_1 \le t_2$). This violates serializability because $T_a$ (already committed) should have read $T_b$'s write. 

\sysname uses leases to avoid this scenario. A validator in \sysname obtains a periodically renewed lease from storage shards (from at least {\em f+1} replicas within each shard) to validate transactions with an commit timestamp $< t_{lease}$. The primary waits for its local clock to advance past $t_{lease}$ before servicing read-write transaction requests for its shard. All outstanding read-write transactions with commit timestamps $< t_{lease}$ can be either aborted or proposed to commit at a timestamp $> t_{lease}$.
%In all failure scenarios (client, primary, backup replica or some combination of the three) a decision can be made on any outstanding transaction and service can be resumed as long as a majority of replicas ($f+1$) of all shards are available.
%\subsection{Scalability}
